Time Course MechInterp: Analyzing the Evolution of Components and Knowledge in Large Language Models

Understanding how large language models (LLMs) acquire and store factual knowledge is crucial for enhancing their interpretability and reliability. In this work, we analyze the evolution of factual knowledge representation in the OLMo-7B model by tracking the roles of its attention heads and feed forward networks (FFNs) over the course of pre-training. We classify these components into four roles: general, entity, relation-answer, and fact-answer specific, and examine their stability and transitions. Our results show that LLMs initially depend on broad, general-purpose components, which later specialize as training progresses. Once the model reliably predicts answers, some components are repurposed, suggesting an adaptive learning process. Notably, attention heads display the highest turnover. We also present evidence that FFNs remain more stable throughout training. Furthermore, our probing experiments reveal that location-based relations converge to high accuracy earlier in training than name-based relations, highlighting how task complexity shapes acquisition dynamics. These insights offer a mechanistic view of knowledge formation in LLMs.

==> chapters/part-6-discussion.tex <==
Our analysis offers a comprehensive view of how OLMo-7B processes and refines factual knowledge during pretraining by examining the roles of its attention heads and FFNs. We uncover distinct patterns of specialization and stability that underpin effective knowledge retention and retrieval.

\paragraph{Evolution and Specialization of Components}
Early in training, attention heads function as general-purpose units, generating broad, context-independent representations and exhibiting high stability (as indicated by strong IoU with the final model). Over time, however, specialized heads—such as proper entity, relation-answer, and answer-specific—begin to emerge to support more precise fact retrieval. Notably, answer-specific heads display the highest turnover, reflecting a dynamic reallocation of resources as the model consolidates its understanding. In contrast, FFNs remain remarkably stable throughout training, serving primarily to refine the representations established by the attention heads.

\paragraph{Stability, Hierarchical Learning, and Task Complexity}
Our IoU and head count analyses reveal a hierarchical learning process. General attention heads form a stable foundation early on, while specialized heads emerge later, suggesting that foundational representations are established first and then refined for task-specific needs. Moreover, name-based relations (e.g., BOOKS\_WRITTEN, COMPANY\_CEO) require more training and exhibit more frequent role transitions in specialized heads compared to location-based relations (e.g., COUNTRY\_CAPITAL\_CITY, CITY\_IN\_COUNTRY), underscoring the greater complexity of these tasks.

\paragraph{Role Switching and Transition Dynamics}
A Markov chain analysis of role transitions further clarifies these dynamics. General heads tend to persist in their roles, while answer-specific heads frequently alternate between relation-answer and deactivated states—with deactivated heads rarely reactivating. This largely irreversible specialization process has important implications for model interpretability, as early pruning may permanently impair performance. Meanwhile, the stable behavior of FFNs reinforces their role in fine-tuning and maintaining robust representations.

In summary, OLMo-7B employs a complementary strategy: dynamic, adaptive specialization in attention heads enables nuanced factual processing, while consistently stable FFNs refine and support these evolving representations.



